Reflections on Visualization in Motion for Fitness Trackers

In this paper, we reflect on our past work towards understanding how to design visualizations for fitness trackers that are used in motion. We have coined the term "visualization in motion" for visualizations that are used in the presence of relative motion between a viewer and the visualization. Here, we describe how visualization in motion is relevant to sports scenarios. We also provide new data on current smartwatch visualizations for sports and discuss future challenges for visualizations in motion for fitness tracker.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> response_letter.tex <==
Dear Dr. Mencarini, dear associate chairs, dear reviewers,

We thank all of you for your reviewing and your detailed comments. Below we respond to all comments.

In this minor revision, we highlighted the different form factors and cited the two recommended references to supplement our research agenda, we shortened the caption of Figure 1, we added a Figure 3 in Section 3.3 to help reading, and we moved Section 4.2 to the related work section (now Section 2.4).

Lijie Yao, on behalf of all authors

-----------------------   METAREVIEW   ---------------------------
The reviewers consider the idea interesting (R1) and relevant to discuss in the workshop (R2).
R1 considers the paper to clearly written and well referenced (R1).
--- Response: We thank all reviewers for their careful reviewing, thoughtful comments, and helpful references.

R2 wishes that the authors would better highlight the position of their work within the larger domain of wearable sports displays, and provides relevant references – I think this could be easily added in one sentence acknowledging these other types of displays exist and would be interesting future work to expand the scope to include them.
--- Response: We highlighted the position of our work in two places: in the section "Fitness tracker Visualizations (2.2) and Display types (4.3) 

I agree with R1, that the content of 3.3 would be much clearer if presented in table format. 
--- Response: We also agree with R1's comment that the content of Section 3.3 would be more readable if presented in table/figure format. We have added a new Figure 3 in Section "3.3-Data Types Representations" to help readers understand the numbers better. The figure shows the average number of representation types on each sports watch face. We have also added the average number of charts or charts combined with text and/or icon representations in the text.

-----------------------   R1   ---------------------------
I was left wondering, could the related work presented in the chapter 4.3 be included in the literature review (Chapter 2). 
--- Response: We moved Section 4.3 to the literature review, now it is Section 2.4.

The chapter 3.3 was a bit difficult to read for me personally, I wonder could it be shared as a table or other figure ? 

--- Response: We have added Figure 3 for Section "3.3-Data Types Representations". Please see our response in the meta review.

The examples are good additions (e.g. Icon+ text). I also didn’t at first realise you limited the analysis to the 42 sport watches, not all the faces, this could be repeated in the 3.2 chapter for clarity. 
--- Response: We now point out that our analysis was about 42 sport watches in Section 3.2, first paragraph, last sentence -- "We present our findings from analyzing 42 sports watch faces in the following."

There is a lot of repetition in the 2.1 chapter and the figure caption.
--- Response: Yes, we agree that the caption of Figure 2.1 is repetitive. We shortened it by cutting the repeated description.

-----------------------   R2   ---------------------------
However, I am a bit confused about the scope of the agenda in terms of form factors and visual modalities that the agenda directs attention to. The authors primarily focus on smartwatch form factors with conventional displays. I believe such an agenda would be more inclusive if it highlights different form factors such as smart clothing or visual modalities such as dynamic textile displays. For instance, [1] proposes a design space for wearable displays including a variety of display modalities that can be considered in this agenda. Also, different form factors with larger display surfaces are suggested to increase the glanceability of the information in a running context [2]. I suggest authors include these aspects in the proposed agenda for providing a broader exploration space about visualisation in motion for fitness.
--- Response: We highlighted the position of our work in two places: in Section 2.2 "Fitness tracker Visualizations and Section 4.3 "Display types."



-------------------------------------------------------------------------------------------------------


